Binary DAD-Net: Binarized Driveable Area Detection Network for Autonomous Driving

Driveable area detection is a key component for various applications in the field of autonomous driving (AD), such as ground-plane detection, obstacle detection and maneuver planning. Additionally, bulky and over-parameterized networks can be easily forgone and replaced with smaller networks for faster inference on embedded systems. The driveable area detection, posed as a two class segmentation task, can be efficiently modeled with slim binary networks. This paper proposes a novel binarized driveable area detection network (binary DAD-Net), which uses only binary weights and activations in the encoder, the bottleneck, and the decoder part. The latent space of the bottleneck is efficiently increased (x32 -> x16 downsampling) through binary dilated convolutions, learning more complex features. Along with automatically generated training data, the binary DAD-Net outperforms state-of-the-art semantic segmentation networks on public datasets. In comparison to a full-precision model, our approach has a x14.3 reduced compute complexity on an FPGA and it requires only 0.9MB memory resources. Therefore, commodity SIMD-based AD-hardware is capable of accelerating the binary DAD-Net.

==> data/backup/backup_30_tdg.tex <==
% The training data generator (TDG), proposed by Mayr \etal \cite{Mayr.01.10.201805.10.2018} automatically labels ground truth data for the task of drivable area segmentation. We adopt this approach as it presents a alternative to the costly manual labeling of the image data on a pixel-level. Although, the data provided by Cityscapes is impressive and very accurate we would like to investigate how the manual training data influences the performance. The automatic labeling allows us to quickly change to other datasets that expose technical (resolution of camera, field of view) and environmental (weather, lightning conditions, street types) domain shifts..
% We apply the four step stereo-vision based TDG \cite{Mayr.01.10.201805.10.2018} to label the training data. 
% The system takes image pairs of a stereo camera as input and computes the corresponding disparity map. Then, a row-wise histogram of the disparity values is created resulting in the v-disparity map. This mapping allows for an easy determination of the drivable area since it is the major horizontal plane in 3D space. Hence, it can be described by a linear function of disparity $d$ and image row coordinate $v$:
% $$f_{DA}(d,v)$$.
% We initialize the linear model based on samples of the bottom area of the image, as the probability of seeing the ground plane there is the highest. Afterwards, we continue to iteratively refine the model in a least-squares fashion by adding samples that satisfy it within a narrow threshold. As soon as the final model is determined, the disparity map can be thresholded in a row-wise manner and every pixel with a disparity that aligns with $f(d,v)$ can be interpreted as being part of the drivable area. 
% Finally, the automatic ground plane annotation is denoised and ready to train a BinaryNet.
% As already mentioned, the TDG can be used to automatically label any custom stereo based images as \cite{Mayr.01.10.201805.10.2018} showed that the approach works across datasets and networks. However, in this paper, CityScapes images are used as it allows us to do a proper comparison between manually and automatically labeled data. In the case that we train on TDG labeled data, we only use manually labeled data in the validation phase.

==> slide.tex <==
Binary DAD is inspired by autoencoder-based networks with skip-connections and enlarged latent space of the bottleneck.

Binary weights and activations (1-Bit precision) in the encoder, the bottleneck and the decoder part

Binary dilated convolutions and automatic annotations (TDG) allow to learn more complex features and close the gap to full-precision CNNs.

BinaryDAD has a 14.3x reduced computational complexity compared to SotA DeepLab.

==> tables/scoremap.tex <==
%night scene
%highway-urban
%fig about the training annoataitons 
% \begin{figure}
%     \subfigure[BinDAD]{\includegraphics[width=1.5cm]{img/heat_maps/overlay_xnor_heat_map_fcn_2c.png}
%     \label{fig:first_sub}}
%     \subfigure[no dilation]{\includegraphics[width=1.5cm]{img/heat_maps/overlay_xnor_heat_map_fcn_2c.png}
%     \label{fig:second_sub}}
%     \subfigure[no ASPP]{\includegraphics[width=1.5cm]{img/heat_maps/overlay_xnor_heat_map_fcn_2c.png}
%     \label{fig:third_sub}}
%     \subfigure[BPAC~\cite{CVPR19Zhuang3}]{\includegraphics[width=1.5cm]{img/heat_maps/overlay_xnor_heat_map_fcn_2c.png}
%     \label{fig:fourth_sub}}
%     \subfigure[ABC~\cite{CVPR19Zhuang3}]{\includegraphics[width=1.5cm]{img/heat_maps/overlay_xnor_heat_map_fcn_2c.png}
%     \label{fig:fourth_sub}}
% \end{figure}
